Hi3DGen: High-fidelity 3D Geometry Generation from Images via Normal Bridging

With the growing demand for high-fidelity 3D models from 2D images, existing methods still face significant challenges in accurately reproducing fine-grained geometric details due to limitations in domain gaps and inherent ambiguities in RGB images. To address these issues, we propose Hi3DGen, a novel framework for generating high-fidelity 3D geometry from images via normal bridging. Hi3DGen consists of three key components: (1) an image-to-normal estimator that decouples the low-high frequency image pattern with noise injection and dual-stream training to achieve generalizable, stable, and sharp estimation; (2) a normal-to-geometry learning approach that uses normal-regularized latent diffusion learning to enhance 3D geometry generation fidelity; and (3) a 3D data synthesis pipeline that constructs a high-quality dataset to support training. Extensive experiments demonstrate the effectiveness and superiority of our framework in generating rich geometric details, outperforming state-of-the-art methods in terms of fidelity. Our work provides a new direction for high-fidelity 3D geometry generation from images by leveraging normal maps as an intermediate representation.

==> tables/equations.tex <==
\newcommand{\normal}{\boldsymbol{n}}
\newcommand{\point}{\boldsymbol{x}}

%\resizebox{0.48\textwidth}{!}{
    %\large
\renewcommand{\arraystretch}{1.3}
    \begin{tabular}{llll}
        \toprule
        Notation & Example\\
        \midrule
         Fraction &  $\frac{1}{a}$ \\
         Max & $\max (a, 0 )$ \\
         Dimension & $\boldsymbol{x} \in \mathbb{R}^3$ \\
         Argmax  & $\mathop{\arg\max}_{a} f(ax)$ \\
         cos & $\cos(x)$ \\
         Hat/tilde & $\hat{\boldsymbol{x}}, \tilde{\boldsymbol{x}}$ \\
         Tensor operation & $\otimes$, \quad $\circ$, \quad $\odot$ \\ 
         Sum & $\sum_{i=1}^{N} x_i$ \\
         Approximation & $f(x) \approx g(x)$ \\
         Around & $\sim$100 \\
         Product & $\prod_{i=1}^{N} x_i$ \\
         Integral & $\int_{-\infty}^{+\infty} x_i$ \\
         Gradient & $\boldsymbol{n}(n) = \nabla o(\boldsymbol{x})/\|\nabla o(\boldsymbol{x})\|_2$ \\
         Parallel & $\mathcal{L} = \sum \| x_i - \hat{x}_i \|^2_2$ \\
         Set & $\{I_i | i=1,\dots, N \}$ \\
        \bottomrule
    \end{tabular}
%    }



==> tables/greek_letters.tex <==
    \resizebox{0.48\textwidth}{!}{
    \large
    \begin{tabular}{clclclclc}
        \toprule
        Symbol & \LaTeX  & Symbol & \LaTeX & Symbol & \LaTeX\\
        \midrule
$\alpha  $ & \textbackslash alpha   & $\kappa $ & \textbackslash kappa  & $\psi    $  & \textbackslash psi    \\
$\beta   $ & \textbackslash beta    & $\lambda$ & \textbackslash lambda & $\rho    $  & \textbackslash rho    \\
$\chi    $ & \textbackslash chi     & $\mu    $ & \textbackslash mu     & $\sigma  $  & \textbackslash sigma  \\
$\delta  $ & \textbackslash delta   & $\nu    $ & \textbackslash nu     & $\tau    $  & \textbackslash tau    \\
$\epsilon$ & \textbackslash epsilon & $ o     $ & \textbackslash o      & $\theta  $  & \textbackslash theta  \\
$\eta    $ & \textbackslash eta     & $\omega $ & \textbackslash omega  & $\upsilon$  & \textbackslash upsilon\\
$\gamma  $ & \textbackslash gamma   & $\phi   $ & \textbackslash phi    & $\xi     $  & \textbackslash xi     \\
$\iota   $ & \textbackslash iota    & $\pi    $ & \textbackslash pi     & $\zeta   $  & \textbackslash zeta   \\
\midrule
$ \digamma   $ & \textbackslash digamma    & $ \Delta $ & \textbackslash digamma    & $ \Theta   $  & \textbackslash Theta  \\
$ \varepsilon$ & \textbackslash varepsilon & $ \Gamma $ & \textbackslash varepsilon & $ \Upsilon $  & \textbackslash Upsilon\\
$ \varkappa  $ & \textbackslash varkappa   & $ \Lambda$ & \textbackslash varkappa   & $ \Xi      $  & \textbackslash Xi     \\
$ \varphi    $ & \textbackslash varphi     & $ \Omega $ & \textbackslash varphi     &               &         \\
$ \varpi     $ & \textbackslash varpi      & $ \Phi   $ & \textbackslash varpi      & $ \aleph   $  & \textbackslash aleph  \\
$ \varrho    $ & \textbackslash varrho     & $ \Pi    $ & \textbackslash varrho     & $ \beth    $  & \textbackslash beth   \\
$ \varsigma  $ & \textbackslash varsigma   & $ \Psi   $ & \textbackslash varsigma   & $ \daleth  $  & \textbackslash daleth \\
$ \vartheta  $ & \textbackslash vartheta   & $ \Sigma $ & \textbackslash vartheta   & $ \gimel   $  & \textbackslash gimel  \\
        \bottomrule
    \end{tabular}
    }



==> tables/ours_version_weg.tex <==

\begin{table}
    \centering
    \begin{tabular}{ccccccccccll} 
         \toprule
         Version&  Bowl&  Buddha&  Bunny&  Cup&  Die&  Hippo&  House&  Owl&  Queen&Squirrel &Ave.\\ 
         \midrule
         baseline &  35.17&  22.33&  33.69&  75.43&  40.06&  28.50 &  37.85&  29.37&  27.68& 29.89& 35.997
\\ 
         + Dual-Stream &  44.27&  20.02&  33.67&  26.00 &  30.51&  23.16&  36.15&  28.84&  28.34& 24.24&29.52
\\
         + Dual-Stream + noise injection &  &  &  &  &  &  &  &  &   &   &  
\\ 
         +Dual-Stream + noise injection + D.S.T &  34.55&  21.13&  30.45&  17.47&  27.20 &  24.64&  34.58&  25.15&  26.82& 24.29&26.628
\\
    \end{tabular}
    \caption{Table 3. Evaluation on Luces-MV (Mean Angular Errors in degrees). }
    \label{tab:my_label}
\end{table}

==> tables/ours_version_woeg.tex <==

\begin{table}
    \centering
    \begin{tabular}{ccccccccccll} 
         \toprule
         versino&  Bowl&  Buddha&  Bunny&  Cup&  Die&  Hippo&  House&  Owl&  Queen&Squirrel &Ave.\\ 
         \midrule
        
         v1.0&  15.72&  16.03&  18.08&  39.85&  10.67&  25.37&  37.70 &  17.49&  18.50 & 25.66&22.507
\\ 
         + Dual-Stream&  26.90 &  14.17&  18.84&  27.68&  13.52&  21.57&  36.38&  19.56&  18.52& 22.04&21.918
\\
         + Dual-Stream + noise injection &  &  &  &  &  &  &  &  &   &   & 
\\ 
         +Dual-Stream + noise injection + D.S.T &  19.26&  15.96&  22.68&  29.81&  13.05&  24.18&  34.08&  18.96&  18.45& 21.94&21.837
\\
    \end{tabular}
    \caption{Table 3. Evaluation on Luces-MV (Mean Angular Errors in degrees). }
    \label{tab:my_label}
\end{table}

==> tables/two_subtables.tex <==
\newcommand{\PSNRT}{PSNR\xspace}
\newcommand{\VQM}{HDR-VQM\xspace}
\newcommand{\VDP}{HDR-VDP2\xspace}
\newcommand{\LowExposure}{Low-Exposure\xspace}
\newcommand{\MiddleExposure}{Middle-Exposure\xspace}
\newcommand{\HighExposure}{High-Exposure\xspace}
\newcommand{\AllExposure}{All-Exposure\xspace}

\makebox[\textwidth]{\small (a) Results on dataset A.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & \Scnd{40.00} & 73.70 & \Scnd{40.04} & \Scnd{70.08} & \Scnd{40.02} & 71.89 & \Scnd{76.22} 
                  & \Scnd{39.61} & 73.24 & \Frst{39.67} & \Frst{73.24} & \Frst{40.01} & 67.90 & \Frst{39.77} & 70.37 & 79.55 \\
    Method B      & 34.54 & 80.22 & 39.25 & 65.96 & 36.90 & 73.09 & 65.33 
                  & 36.51 & 77.78 & 37.45 & 69.79 & 39.02 & 64.57 & 37.66 & 70.71 & 70.13 \\
    Method C  & 39.79 & \Scnd{81.02} & 39.96 & 67.25 & 39.88 & \Scnd{74.13} & 73.84 
                  & 39.48 & \Scnd{78.13} & 38.43 & 70.08 & 39.60 & \Scnd{67.94} & 39.17 & \Scnd{72.05} & \Scnd{80.70} \\
    Ours          & \Frst{41.95} & \Frst{81.03} & \Frst{40.41} & \Frst{71.27} & \Frst{41.18} & \Frst{76.15} & \Frst{78.84}
                  & \Frst{40.00} & \Frst{78.66} & \Scnd{39.27} & \Scnd{73.10} & \Scnd{39.99} & \Frst{69.99} & \Scnd{39.75} & \Frst{73.92} & \Frst{82.87} \\
    \bottomrule
\end{tabular}
}

\vspace{0.5em}
\makebox[\textwidth]{\small (b) Results on dataset B.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & 37.73 & 74.05 & 45.71 & 66.67 & 41.72 & 70.36 & 85.33 
                  & 37.53 & 72.03 & 36.38 & 65.37 & 34.73 & 62.24 & 36.21 & 66.55 & 84.43 \\
    Method B      & 36.41 & 85.68 & \Scnd{49.89} & \Scnd{69.90} & 43.15 & 77.79 & 78.92 
                  & 36.43 & 77.74 & 39.80 & \Scnd{67.88} & \Scnd{43.03} & \Scnd{64.74} & 39.75 & \Scnd{70.12} & 87.93 \\
    Method C  & \Scnd{39.94} & \Scnd{86.77} & 49.49 & 69.04 & \Scnd{44.72} & \Scnd{77.91} & \Scnd{87.16} 
                  & \Scnd{38.34} & \Scnd{78.04} & \Scnd{41.21} & 66.07 & 42.66 & 64.01 & \Scnd{40.74} & 69.37 & \Scnd{89.36}\\
    Ours          & \Frst{40.83} & \Frst{86.84} & \Frst{50.10} & \Frst{71.33} & \Frst{45.46} & \Frst{79.09} & \Frst{87.40} 
                  & \Frst{38.77} & \Frst{78.11} & \Frst{41.47} & \Frst{68.49} & \Frst{43.24} & \Frst{65.08} & \Frst{41.16} & \Frst{70.56} & \Frst{89.56}\\
    \bottomrule
\end{tabular}
}

